Cross-Modal Generalization: Learning in Low Resource Modalities via Meta-Alignment

The natural world is abundant with concepts expressed via visual, acoustic, tactile, and linguistic modalities. Much of the existing progress in multimodal learning, however, focuses primarily on problems where the same set of modalities are present at train and test time, which makes learning in low-resource modalities particularly difficult. In this work, we propose algorithms for cross-modal generalization: a learning paradigm to train a model that can (1) quickly perform new tasks in a target modality (i.e. meta-learning) and (2) doing so while being trained on a different source modality. We study a key research question: how can we ensure generalization across modalities despite using separate encoders for different source and target modalities? Our solution is based on meta-alignment, a novel method to align representation spaces using strongly and weakly paired cross-modal data while ensuring quick generalization to new tasks across different modalities. We study this problem on 3 classification tasks: text to image, image to audio, and text to speech. Our results demonstrate strong performance even when the new target modality has only a few (1-10) labeled samples and in the presence of noisy labels, a scenario particularly prevalent in low-resource modalities.

==> CVPR2021_Meta Alignment/bold_symbols.tex <==
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bdot}{\mathbf{cdot}}

==> CVPR2021_Meta Alignment/figs/alg.tex <==
\begin{figure*}
    \begin{minipage}{\linewidth}
    \vspace{-2mm}
    \begin{algorithm}[H]
    \caption{\textsc{CroMA}: \namel}
    \begin{algorithmic}
    \State Initialize meta-alignment encoders $e_s^\textrm{meta}$ and $e_t^\textrm{meta}$, meta-classifier $\phi^\textrm{meta}$.
    \For{iteration = $1,2,\dots$}
        \State Sample alignment task $\mathcal{T}_{a}$ with train $\mathcal{D}^{\mathcal{T}_{a}}_{\textrm{train}}$ and test data $\mathcal{D}^{\mathcal{T}_{a}}_{\textrm{test}}$ of pairs $\{ x_s, x_t \}$.
        \State Initialize $e_s := e_s^\textrm{meta}, e_t := e_t^\textrm{meta}$ and compute alignment loss~\eqref{align_eq} on train data $\mathcal{D}^{\mathcal{T}_{a}}_{\textrm{train}}$.
        \State Compute $\wt{e}_s$ and $\wt{e}_t$ after gradient updates using alignment loss wrt $e_s$ and $e_t$.
        \State Update meta-alignment encoders $e_s^\textrm{meta} \leftarrow e_s^\textrm{meta} + \epsilon (\wt{e}_s - e_s^\textrm{meta})$, $e_t^\textrm{meta} \leftarrow e_t^\textrm{meta} + \epsilon (\wt{e}_t - e_t^\textrm{meta})$.
        \State Sample source modality task $\mathcal{T}_{s}$ with train $\mathcal{D}^{\mathcal{T}_{s}}_{\textrm{train}}$ and test data $\mathcal{D}^{\mathcal{T}_{s}}_{\textrm{test}}$ of pairs $\{ x_s, y_s \}$.
        \State Initialize $\phi := \phi^\textrm{meta}$ and compute classification loss on train data $\mathcal{D}^{\tau_s}_{\textrm{train}}$.
        \State Compute $\wt{\phi}$ after gradient updates using classification loss wrt $\phi$.
        \State Update meta-classifier $\phi^\textrm{meta} \leftarrow \phi^\textrm{meta} + \epsilon (\wt{\phi} - \phi^\textrm{meta})$.
    \EndFor
    \end{algorithmic}
    \label{algo}
    \end{algorithm}
    \end{minipage}
    \vspace{-2mm}
\end{figure*}

\iffalse

\begin{algorithm}[H]
\caption{Cross-modality generalization via meta-alignment: TESTING}
\begin{algorithmic}
\State Trained $\phi^*$, the vector of initial classifier meta-parameters.
\State Trained modality encoders $e_1^*$ and $e_2^*$.
\For{iteration = $1,2,\dots$}
  \State Sample task $\tau_2$ from target modality with train $\mathcal{D}^{\tau_2}_{\textrm{train}} = \{ x_s, x_t \}$ and test data $\mathcal{D}^{\tau_2}_{\textrm{test}}$.
  \State Embed data using trained modality encoder into aligned space: $e_2^* (y)$.
  \State Initialize a model $\psi$ on task $\tau_2$ using meta-parameters $\phi^*$.
  \State Compute loss $L_{\tau}$ on train data $\mathcal{D}^{\tau_2}_{\textrm{train}}$ using model.
  \State Compute $\tilde{\psi} = U^m_{\tau_2}(\psi)$, denoting $k$ gradient updates on task $\tau_2$ wrt loss $L_{\tau_2}$.
  \State Update model parameters $\psi^* \leftarrow \psi + \epsilon (\tilde{\psi} - \psi)$.
\EndFor
\State Return performance on target task, measured on test data $\mathcal{D}^{\tau_2}_{\textrm{test}}$ using model parameters $\psi^*$.
\end{algorithmic}
\end{algorithm}

\fi

==> CVPR2021_Meta Alignment/figs/concepts.tex <==
\begin{figure*}[tbp]
\centering
\vspace{-4mm}
\includegraphics[width=\linewidth]{figs/concepts_fig.pdf}
\caption{The $17$ concepts shared across image and audio classification tasks that were used for weak alignment. Note that we only show the images - the audio spectrograms make up the second modality in each weak cluster.\vspace{-4mm}}
\label{concepts}
\end{figure*}

==> CVPR2021_Meta Alignment/figs/first.tex <==
\begin{figure}[tbp]
\centering
\vspace{-2mm}
\includegraphics[width=0.85\linewidth]{figs/first_fig.pdf}
\vspace{-2mm}
\caption{The \textit{cross-modal generalization} paradigm brings discrepancies in both input and output spaces with \textit{new tasks} expressed in \textit{new modalities}. This raises a fundamental question: how can we ensure generalization across modalities despite using separate encoders for different source (image) and target (audio) modalities? This paper studies the minimal supervision required to perform this alignment and succeed in cross-modal generalization.\vspace{-4mm}}
\label{first_fig}
\end{figure}
%We highlight 2 conceptual differences with domain adaptation, transfer learning, and meta/multi-task learning: cross-modal generalization shows 1) high-dimensional, complex, and heterogeneous source and target modalities, and 2) task-discrepancies between source and target modalities.

==> CVPR2021_Meta Alignment/figs/graph.tex <==
\begin{figure}[tbp]
\centering
\vspace{-2mm}
\includegraphics[width=0.7\linewidth]{figs/graph_fig.pdf}
\vspace{-1em}
\caption{One obtains a subset of observed edges through labeled datasets for source modalities $x_s$ and tasks $y_s$ (solid edges). Generalizing to the target modalities $x_t$ and tasks $y_t$ (dotted edge) requires bridging modalities and tasks through alignment (purple).\vspace{-1em}}
\label{graph}
\end{figure}

==> CVPR2021_Meta Alignment/figs/meta.tex <==
\begin{figure*}[tbp]
\centering
\vspace{-6mm}
\includegraphics[width=0.9\linewidth]{figs/meta_fig.pdf}
\vspace{-1em}
\caption{While strong pairs (a) provide exact, one-to-one correspondences across modalities, weak pairs (b) represent coarse semantic groupings which better reflect many-to-many cross-modal mappings and leverage weakly paired multimodal data available on the internet (e.g. videos, image captions). (c) During meta-training, meta-parameters $e_s^\textrm{meta}, e_t^\textrm{meta}, \phi^\textrm{meta}$ are trained using source modality classification tasks $\mathcal{T}_s$ and alignment tasks $\mathcal{T}_a$. Meta-testing uses trained meta-parameters for few-shot generalization to target modality tasks $\mathcal{T}_t$.\vspace{-2mm}}
\label{meta}
\end{figure*}

==> CVPR2021_Meta Alignment/figs/noise.tex <==
\begin{figure}[tbp]
\centering
\includegraphics[width=0.7\linewidth]{figs/noise_fig.pdf}
\vspace{-2mm}
\caption{\name\ is robust to noisy labels in the target modality by using cross-modal information from the source, making it suitable for low-resource modalities with imperfect annotations.\vspace{-4mm}}
\label{noise}
\end{figure}

==> CVPR2021_Meta Alignment/figs/overview.tex <==
\begin{figure}[tbp]
\centering
\vspace{-0mm}
\includegraphics[width=\linewidth]{figs/overview_fig.pdf}
\vspace{-6mm}
\caption{\textit{Meta-alignment} aligns representation spaces while ensuring quick generalization to new tasks using strongly (image and audio) and weakly (video) paired data. This enables generalization to the target (audio) having only seen labeled data in the source (image), as assessed by few-shot classification and alignment tasks.\vspace{-4mm}}
\label{overview_fig}
\end{figure}
% leverages data from abundant source modalities (text) for scarce target modalities (images). To solve this, we propose
% While existing domain adaptation, transfer learning, and meta/multi-task learning approaches are unable to bridge the gap between such heterogeneous input modalities and output tasks, our proposed \textit{meta-alignment} approach allows for efficient generalization to a new low-resource target modality with only a few (1-10) labeled samples.

==> CVPR2021_Meta Alignment/figs/pairs.tex <==
\begin{figure*}[tbp]
\centering
\includegraphics[width=0.9\linewidth]{figs/pairs_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Left}: samples of retrieved images given text recipes. \names\ performs few-shot retrieval of images more accurately than existing alignment approaches. \textbf{Right}: samples of retrieved audio samples given images. Despite being trained only on \textit{weak pairs}, meta-alignment can perform few-shot cross-modal retrieval at fine granularities (e.g. amphibian, automobile).\vspace{-4mm}}
\label{pairs}
\end{figure*}

==> CVPR2021_Meta Alignment/figs/syn.tex <==
\begin{figure}[tbp]
\centering
\includegraphics[width=0.75\linewidth]{figs/syn_fig.pdf}
\vspace{-2mm}
\caption{Supervision learning vs alignment for synthetic data: with more strongly or weakly aligned pairs ($n_{\rm align}$), cross-modal alignment improves upon supervised learning in target tasks.\vspace{-4mm}}
\label{syn}
\end{figure}

==> CVPR2021_Meta Alignment/rl_math.tex <==
% GENL MATH
\newcommand{\Real}{\mathbb{R}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\given}[1][]{\:#1\vert\:}
\newcommand{\givenb}{\:\middle\vert\:}
\newcommand{\suchthat}{\:\vert\:}
\newcommand{\grad}{\nabla}
\newcommand{\evalat}[1]{\big\rvert_{#1}}

% STATISTICS
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Ea}[1]{\E\left[#1\right]}
\newcommand{\Eb}[2]{\E_{#1}\left[#2\right]}
\newcommand{\Vara}[1]{\Var\left[#1\right]}
\newcommand{\Varb}[2]{\Var_{#1}\left[#2\right]}
\newcommand{\lone}[1]{\norm{#1}_1}
\newcommand{\Prob}[1]{\operatorname{Pr}\left[#1\right]}

% NORMS
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\abs}{|}{|}
\newcommand{\pospart}[1]{\abs{#1}^+}
\DeclarePairedDelimiter{\lrbrack}{[}{]}
\DeclarePairedDelimiter{\lrbrace}{ \{ }{ \} }
\DeclarePairedDelimiter{\lrparen}{(}{)}
\DeclarePairedDelimiter{\lrang}{\langle}{\rangle}
\newcommand{\infnorm}[1]{\norm{#1}_{\infty}}
\newcommand{\normone}[1]{\norm{#1}_1}

% MDP
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\adv}{\mathbb{A}}
\newcommand{\rhopi}{\rho_{\pi}}
\newcommand{\Qpi}{\ensuremath{Q^{\pi}}}
\newcommand{\Api}{\ensuremath{A^{\pi}}}
\newcommand{\Vpi}{\ensuremath{V^{\pi}}}
\newcommand{\Qstar}{\ensuremath{Q^{*}}}
\newcommand{\Astar}{\ensuremath{A^{*}}}
\newcommand{\Vstar}{\ensuremath{V^{*}}}

% DIVERGENCE
\newcommand{\kl}[2]{D_{KL}\left[#1 ~ \| ~ #2\right]}
\newcommand{\tv}[2]{D_{TV}(#1 \ \| \ #2)}

% MISC
\newcommand{\tdlam}{TD($\lambda$)}
\newcommand{\tdzero}{TD($0$)}
\newcommand{\tdone}{TD($1$)}
\newcommand{\lstdlam}{LSTD($\lambda$)}
\newcommand{\lstdzero}{LSTD($0$)}
\newcommand{\lstdone}{LSTD($1$)}
\newcommand{\brmlam}{BRM($\lambda$)}
\newcommand{\brmzero}{BRM($0$)}
\newcommand{\brmone}{BRM($1$)}
\newcommand{\lspelam}{LSPE($\lambda$)}
\newcommand{\lspezero}{LSPE($0$)}
\newcommand{\lspeone}{LSPE($1$)}
\newcommand{\qlrn}{$Q$-learning}
\newcommand{\qfcn}{$Q$-function}
\newcommand{\sarsalam}{SARSA($\lambda$)}
\newcommand{\gaelam}{GAE($\lambda$)}
\newcommand{\sarsazero}{SARSA($0$)}
\newcommand{\watq}{Watkins' $Q$-learning}
\newcommand{\myint}[1]{\int \! \! \mathrm{d} #1 \ }


==> CVPR2021_Meta Alignment/tables/image_audio.tex <==
\begin{table*}[t]
\fontsize{9}{11}\selectfont
\centering
\caption{Performance on text to image generalization on Yummly-28K (top), image to audio concept classification from CIFAR to ESC-50 (middle), and text to speech generalization on the Wilderness dataset (bottom). \name\ is on par and sometimes outperforms the oracle target modality meta-learning approach that has seen thousands of labeled target samples, and also outperforms existing unimodal, domain adaptation, and cross-modal baselines. \#Target (labels) denotes the number of target modality samples and labels used during meta-training.}
\vspace{-1em}
%\caption{Performance on text to speech generalization on the Wilderness dataset. \name\ outperforms the oracle few-shot speech baseline that has seen thousands of labeled speech samples and the existing unimodal baselines. \#Speech (labeled) denotes the number of speech samples and labels used during meta-training.}
\setlength\tabcolsep{2.0pt}
\begin{tabular}{C{1.7cm} L{1.9cm} L{5.2cm} || *{3}{C{1.6cm}} C{2.7cm}}
\Xhline{3\arrayrulewidth}
{\sc Task} & {\sc Type} & {\sc Approach}  & {\sc 1-Shot} & {\sc 5-Shot} & {\sc 10-Shot} & {\sc \#Target (labels)}\\
\Xhline{0.5\arrayrulewidth}
\multirow{6}{*}{\shortstack{{\color{gg}Text}\\(Yummly)\\$\downarrow$\\{\color{rr}Image}\\(Yummly)}} & \multirow{2}{*}{Unimodal} & Pre-training~\cite{baevski2019effectiveness,devlin2018bert} & $33.1 \pm 2.8$ & $36.4 \pm 3.5$ & $49.0 \pm 3.8$ & $0(0)$\\
& & Unsup. meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} (reconstruct) & $37.4 \pm 0.6$ & $41.7 \pm 3.7$ & $49.0 \pm 1.0$ & $5131 (0)$ \\
\cline{2-7}
& \multirow{3}{*}{Cross-modal} & Align + Classify~\cite{cicek2019unsupervised,DBLP:journals/corr/abs-1711-03213,DBLP:journals/corr/RajNT15a,tzeng2017adversarial,10.5555/2283516.2283652} & $37.1 \pm 3.0$ & $40.0 \pm 2.7$ & $47.8 \pm 6.6$ & $5131 (0)$ \\
& & Align + Meta Classify~\cite{sahoo2019metalearning} & $39.4 \pm 2.5$ & $40.0 \pm 2.3$ & $48.8 \pm 7.8$ & $5131 (0)$ \\
& & \textbf{\names\ (ours)} & $\mathbf{39.7 \pm 1.3}$ & $\mathbf{47.1 \pm 3.3}$ & $\mathbf{51.1 \pm 2.1}$ & $5131 (0)$ \\
\cline{2-7}
& \multirow{1}{*}{Oracle} & Within modality generalization~\cite{finn2017model,nichol2018reptile} & $38.9 \pm 2.1$ & $42.1 \pm 1.4$ & $47.9 \pm 5.6$ & $5131 (5131)$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{C{1.7cm} L{1.9cm} L{5.2cm} || *{3}{C{1.6cm}} C{2.7cm}}
\Xhline{3\arrayrulewidth}
\multirow{7}{*}{\shortstack{{\color{gg}Image}\\(CIFAR)\\$\downarrow$\\{\color{rr}Audio}\\(ESC-50)}} & \multirow{3}{*}{Unimodal} & Pre-training~\cite{baevski2019effectiveness,devlin2018bert} & $44.2 \pm 0.8$ & $72.3 \pm 0.3$ & $77.4 \pm 1.7$ & $0(0)$\\
& & Unsup. meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} (reconstruct) & $36.3 \pm 1.8$ & $67.3 \pm 0.9$ & $76.6 \pm 2.1$ & $920 (0)$ \\
& & Unsup. meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} (weak labels) & $45.6 \pm 1.3$ & $74.2 \pm 0.3$ & $83.7 \pm 0.1$ & $920 (0)$ \\
\cline{2-7}
& \multirow{3}{*}{Cross-modal} & Align + Classify~\cite{cicek2019unsupervised,DBLP:journals/corr/abs-1711-03213,DBLP:journals/corr/RajNT15a,tzeng2017adversarial,10.5555/2283516.2283652} & $45.3 \pm 0.8$ & $73.9 \pm 2.1$ & $78.8 \pm 0.1$ & $920 (0)$ \\
& & Align + Meta Classify~\cite{sahoo2019metalearning} & $47.2 \pm 0.3$ & $77.1 \pm 0.7$ & $80.4 \pm 0.0$ & $920 (0)$ \\
& & \textbf{\names\ (ours)} & $\mathbf{47.5 \pm 0.2}$ & $\mathbf{85.9 \pm 0.7}$ & $\mathbf{92.7 \pm 0.4}$ & $920 (0)$ \\
\cline{2-7}
& \multirow{1}{*}{Oracle} & Within modality generalization~\cite{finn2017model,nichol2018reptile} & $45.9 \pm 0.2$ & $89.3 \pm 0.4$ & $94.5 \pm 0.3$ & $920 (920)$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{C{1.7cm} L{1.9cm} L{5.2cm} || *{3}{C{1.6cm}} C{2.7cm}}
\Xhline{3\arrayrulewidth}
\multirow{10}{*}{\shortstack{{\color{gg}Text}\\(Wilderness)\\$\downarrow$\\{\color{rr}Speech}\\(Wilderness)}} & \multirow{2}{*}{Unimodal} & Pre-training~\cite{baevski2019effectiveness,devlin2018bert} & $55.2 \pm 8.6$ & $73.1 \pm 3.4$ & $84.3 \pm 0.1$ & $0 (0)$\\
& & Unsup. meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} (reconstruct) & $61.5 \pm 4.4$ & $83.5 \pm 4.0$ & $88.5 \pm 2.1$ & $4395 (0)$\\
%& Unsup. meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} (weak labels) & $ \pm $ & $ \pm $ & $ \pm $ & $4395 (0)$\\
\cline{2-7}
& \multirow{4}{*}{\shortstack[l]{Domain\\Adaptation}} & Shared~\cite{DBLP:journals/corr/HuhAE16} & $55.6 \pm 10.2$ & $75.2 \pm 8.4$ & $81.9 \pm 3.9$ & $4395 (0)$\\
& & Shared + Align~\cite{jawanpuria2020geometry} & $59.7 \pm 7.6$ & $78.4 \pm 6.2$ & $84.3 \pm 1.5$ & $4395 (0)$\\
& & Shared + Domain confusion~\cite{DBLP:journals/corr/TzengHZSD14} & $59.5 \pm 7.2$ & $76.3 \pm 9.4$ & $83.9 \pm 1.8$ & $4395 (0)$\\
& & Shared + Target labels~\cite{DBLP:journals/corr/abs-0907-1815} & $57.3 \pm 9.3$ & $76.2 \pm 8.4$ & $84.0 \pm 1.9$ & $4395 (4395)$\\
\cline{2-7}
& \multirow{3}{*}{Cross-modal} & Align + Classify~\cite{cicek2019unsupervised,DBLP:journals/corr/abs-1711-03213,DBLP:journals/corr/RajNT15a,tzeng2017adversarial,10.5555/2283516.2283652} & $61.1 \pm 6.0$ & $74.8 \pm 2.1$ & $86.2 \pm 0.7$ & $4395 (0)$\\
& & Align + Meta Classify~\cite{sahoo2019metalearning} & $65.6 \pm 6.1$ & $89.9 \pm 1.5$ & $93.0 \pm 0.5$ & $4395 (0)$\\
& & \textbf{\names\ (ours)} & $\mathbf{67.9 \pm 6.6}$ & $\mathbf{90.6 \pm 1.5}$ & $\mathbf{93.2 \pm 0.2}$ & $4395 (0)$\\
\cline{2-7}
& \multirow{1}{*}{Oracle} & Within modality generalization~\cite{finn2017model,nichol2018reptile} & $61.3 \pm 11.2$ & $77.0 \pm 0.3$ & $87.5 \pm 0.6$ & $4395 (4395)$\\ % $67.7 \pm 6.6$ & $86.6 \pm 0.8$ & $91.4 \pm $ & $4395 (4395)$\\
\Xhline{3\arrayrulewidth}
\end{tabular}

\label{tts}
\vspace{0mm}
\end{table*}

\iffalse
\begin{table}[]
\caption{Image-Audio Results: no\_meta\_tri is our proposed approach without any meta learning, meta\_1\_tri is our proposed approach with meta learning applied to only the classifier, reptile\_audio is unimodal meta learning, reptile\_cos is our proposed approach with our alignment loss function replaced with the cosine similarity loss, reptile\_tri is our proposed approach that uses triplet loss, lstm\_ae is the unsupervised unimodal model}
\begin{tabular}{lrr}
                   & \multicolumn{1}{l}{mean} & \multicolumn{1}{l}{stdev} \\
no\_meta\_tri k1   & 0.27847                  & 0.002741471624            \\
no\_meta\_tri k5   & 0.75375                  & 0.005417922931            \\
no\_meta\_tri k10  & 0.89296                  & 0.004698746878            \\
meta\_1\_tri k1    & 0.27847                  & 0.002741471624            \\
meta\_1\_tri k5    & 0.75375                  & 0.005417922931            \\
meta\_1\_tri k10   & 0.89296                  & 0.004698746878            \\
reptile\_audio k1  & 0.4588                   & \multicolumn{1}{l}{-}     \\
reptile\_audio k5  & 0.893                    & \multicolumn{1}{l}{-}     \\
reptile\_audio k10 & 0.9449                   & \multicolumn{1}{l}{-}     \\
pretrain k1        & 0.37107                  & 0.006681658144            \\
pretrain k5        & 0.82093                  & 0.009056372833            \\
pretrain k10       & 0.89296                  & 0.004698746878            \\
reptile\_cos k1    & \multicolumn{1}{l}{-}    & \multicolumn{1}{l}{-}     \\
reptile\_cos k5    & 0.7785                   & \multicolumn{1}{l}{-}     \\
reptile\_cos k10   & 0.9058                   & \multicolumn{1}{l}{-}     \\
reptile\_tri k1    & 0.4127875                & 0.02109498502             \\
reptile\_tri k5    & 0.8275                   & \multicolumn{1}{l}{-}     \\
reptile\_tri k10   & 0.9023166667             & 0.00352443849             \\
lstm\_ae k1        & 0.3566                   & 0.02120429726             \\
lstm\_ae k5        & 0.67055                  & 0.01762682615             \\
lstm\_ae k10       & 0.75358                  & 0.02033441527            
\end{tabular}
\end{table}
\fi

==> CVPR2021_Meta Alignment/tables/image_audio_align.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[t!]
\vspace{-0mm}
\fontsize{9}{11}\selectfont
\caption{\name\ yields better alignment scores than the baselines, indicating that meta-alignment can align new concepts using only \textit{weakly paired data} across image and audio.}
\vspace{-1em}
\setlength\tabcolsep{3.0pt}
\begin{tabular}{l l || c c c c c}
\Xhline{3\arrayrulewidth}
{\sc $K$} & {\sc Experiment} & {\sc R$@1$} \textcolor{gg}{$\uparrow$} & {\sc R$@5$} \textcolor{gg}{$\uparrow$} & {\sc R$@10$} \textcolor{gg}{$\uparrow$} & {\sc Rank} \textcolor{gg}{$\downarrow$} & {\sc Cos.} \textcolor{gg}{$\downarrow$} \\
\Xhline{0.5\arrayrulewidth} % %,	R@5:	%,	R@10: %,	Median Rank: 101
\multirow{3}{*}{$5$} & No align & $1.0\%$ & $2.0\%$ & $5.5\%$ & $101$ & $0.428$\\
& Align & $2.0\%$ & $5.5\%$ & $8.5\%$ & $103$ & $0.272$\\
& \textbf{\names} & $\mathbf{4.0\%}$ & $\mathbf{19.5\%}$ & $\mathbf{39.0\%}$ & $\mathbf{13}$ & $\mathbf{0.003}$\\
\Xhline{0.5\arrayrulewidth}% R@1: 0.5%,	R@5:	3.0%,	R@10: 4.5%
\multirow{3}{*}{$10$} & No align & $0.5\%$ & $3.0\%$ & $4.5\%$ & $101$ & $0.399$\\
& Align & $1.5\%$ & $11.0\%$ & $18.5\%$ & $52$ & $0.222$\\
& \textbf{\names} & $\mathbf{3.5\%}$ & $\mathbf{17.5\%}$ & $\mathbf{35.0\%}$ & $\mathbf{15}$ & $\mathbf{0.004}$\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{image_audio_align}
\vspace{-4mm}
\end{table}

\iffalse

\begin{table*}[t!]
\vspace{-2mm}
\begin{minipage}{.6\linewidth}
\fontsize{9}{11}\selectfont
\caption{\textbf{Left}: \name\ yields better alignment scores than the baselines, indicating that meta-alignment can align new concepts using only weakly paired data. \textbf{Right}: samples of retrieved images given an audio sample. Despite being trained on weak pairs, meta-alignment can perform cross-modal retrieval at fine granularities.}
\setlength\tabcolsep{3.0pt}
\begin{tabular}{l l || c c c c c}
\Xhline{3\arrayrulewidth}
{\sc $K$} & {\sc Experiment} & {\sc R$@1$} \textcolor{gg}{$\uparrow$} & {\sc R$@5$} \textcolor{gg}{$\uparrow$} & {\sc R$@10$} \textcolor{gg}{$\uparrow$} & {\sc Rank} \textcolor{gg}{$\downarrow$} & {\sc Cos.} \textcolor{gg}{$\downarrow$} \\
\Xhline{0.5\arrayrulewidth} % %,	R@5:	%,	R@10: %,	Median Rank: 101
\multirow{3}{*}{$5$} & No align & $1.0\%$ & $2.0\%$ & $5.5\%$ & $101$ & $0.428$\\
& Align & $2.0\%$ & $5.5\%$ & $8.5\%$ & $103$ & $0.272$\\
& \textbf{\names} & $\mathbf{4.0\%}$ & $\mathbf{19.5\%}$ & $\mathbf{39.0\%}$ & $\mathbf{13}$ & $\mathbf{0.003}$\\
\Xhline{0.5\arrayrulewidth}% R@1: 0.5%,	R@5:	3.0%,	R@10: 4.5%
\multirow{3}{*}{$10$} & No align & $0.5\%$ & $3.0\%$ & $4.5\%$ & $101$ & $0.399$\\
& Align & $1.5\%$ & $11.0\%$ & $18.5\%$ & $52$ & $0.222$\\
& \textbf{\names} & $\mathbf{3.5\%}$ & $\mathbf{17.5\%}$ & $\mathbf{35.0\%}$ & $\mathbf{15}$ & $\mathbf{0.004}$\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{image_audio_align}
%
\end{minipage}
\hspace{0mm}
\begin{minipage}{.4\linewidth}
\vspace{2mm}
\includegraphics[width=\linewidth]{figs/pairs_fig.pdf}
\vspace{-6mm}
\end{minipage}

\vspace{-6mm}
\end{table*}

\begin{table*}[!tbp]
\fontsize{9}{11}\selectfont
\centering
\caption{\name\ yields noticeably better alignment metric values than the baseline approach, indicating that meta-alignment is able to align new concepts during meta-test even with weak paired data.}
\setlength\tabcolsep{3.0pt}
\begin{tabular}{l l || c c c c c}
\Xhline{3\arrayrulewidth}
{\sc $k$} & {\sc Experiment} & {\sc R$@1$} \textcolor{gg}{$\uparrow$} & {\sc R$@5$} \textcolor{gg}{$\uparrow$} & {\sc R$@10$} \textcolor{gg}{$\uparrow$} & {\sc Rank} \textcolor{gg}{$\downarrow$} & {\sc Cos.} \textcolor{gg}{$\downarrow$} \\
\Xhline{0.5\arrayrulewidth} % %,	R@5:	%,	R@10: %,	Median Rank: 101
\multirow{3}{*}{$5$} & No alignment & $1.0\%$ & $2.0\%$ & $5.5\%$ & $101$ & $0.4275$\\
& Alignment & \\
& \textbf{\names} & $4.0\%$ & $19.5\%$ & $39.0\%$ & $13$ & $0.0029$\\
\Xhline{0.5\arrayrulewidth}% R@1: 0.5%,	R@5:	3.0%,	R@10: 4.5%
\multirow{3}{*}{$10$} & No alignment & $0.5\%$ & $3.0\%$ & $4.5\%$ & $101$ & $0.3993$\\
& Alignment & \\
& \textbf{\names} & $3.5\%$ & $17.5\%$ & $35.0\%$ & $15$ & $0.0036$\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{image_audio_align}
\vspace{-6mm}
\end{table*}

\fi

==> CVPR2021_Meta Alignment/tables/image_audio_params.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\centering
\caption{Table of hyperparameters for generalization experiments on image to audio task. Batchsize $4/8/16$ indicates the batchsize used for $1/5/10$-shot experiments respectively.\vspace{2mm}}
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{14}{*}{Image Encoder}
& Shared layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-3$\\
& Iterations & $800$\\
& Number of evaluation tasks & 16\\
& Loss Margin & $0.1$\\
& Width Factor & $1.3$ \\
& Number of Layers & $4$ \\
& Blocks Per Layer & $4, 5, 24, 3$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{14}{*}{Audio Encoder}
& Shared layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-3$\\
& Iterations & $800$\\
& Number of evaluation tasks & 16\\
& Loss Margin & $0.1$\\
& Intermediate Pooling Function & Max \\
& Final Pooling Function & Average \\
& Stride & 1 \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{13}{*}{Audio Classifier}
& Num hidden layers & $1$ \\
& Hidden layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-3$\\
& Iterations & $800$\\
& Number of evaluation tasks & 16\\
& Loss & MSE\\
& Teacher forcing rate & $0.5$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-4mm}
\label{image_audio_params}
\end{table}

==> CVPR2021_Meta Alignment/tables/image_audio_wk_align.tex <==
\begin{table*}[t]
\fontsize{9}{11}\selectfont
\centering
\caption{Performance on image to audio concept classification from CIFAR-10 and CIFAR-100 to ESC-50. \name\ is on par with the oracle few-shot audio baseline that has seen a thousand of labeled audio samples and outperforms existing unimodal and cross-modal baselines. \#Audio (labeled) denotes the number of audio samples and labels used during meta-training.}
\setlength\tabcolsep{2.0pt}
\begin{tabular}{l l || c c c c c c c}
\Xhline{3\arrayrulewidth}
{\sc Type} & {\sc Approach}  & {\sc 1-Shot} & {\sc 5-Shot} & {\sc 10-Shot} & {\sc \#Audio (labeled)}\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{Uni} & Unsup. pre-training~\cite{baevski2019effectiveness,devlin2018bert} & $44.2 \pm 0.8$ & $72.3 \pm 0.3$ & $77.4 \pm 1.7$ & $0(0)$\\
& Unsup. meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} (reconstruct) & $36.3 \pm 1.8$ & $67.3 \pm 0.9$ & $76.6 \pm 2.1$ & $920 (0)$ \\
& Unsup. meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} (weak labels) & $45.6 \pm 1.3$ & $74.2 \pm 0.3$ & $83.7 \pm 0.1$ & $920 (0)$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{Cross} & Align + Classify~\cite{cicek2019unsupervised,DBLP:journals/corr/abs-1711-03213,DBLP:journals/corr/RajNT15a,tzeng2017adversarial,10.5555/2283516.2283652} & $45.3 \pm 0.8$ & $73.9 \pm 2.1$ & $78.8 \pm 0.1$ & $920 (0)$ \\
& Align + Meta Classify~\cite{sahoo2019metalearning} & $47.2 \pm 0.3$ & $77.1 \pm 0.7$ & $80.4 \pm 0.0$ & $920 (0)$ \\
& \textbf{\names\ (ours)} & $\mathbf{47.5 \pm 0.2}$ & $\mathbf{85.9 \pm 0.7}$ & $\mathbf{92.7 \pm 0.4}$ & $920 (0)$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{1}{*}{Oracle} & Within modality generalization~\cite{finn2017model,nichol2018reptile} & $45.9 \pm 0.2$ & $89.3 \pm 0.4$ & $94.5 \pm 0.3$ & $920 (920)$ \\
\Xhline{3\arrayrulewidth}
%~\cite{tzeng2017adversarial,cicek2019unsupervised,DBLP:journals/corr/abs-1711-03213,10.5555/2283516.2283652,DBLP:journals/corr/RajNT15a}
%~\cite{sahoo2019metalearning}
%& {\sc \#Images} & {\sc \#Image labels} \\
%{Baseline} & 0.3233 & 0.8094 & 0.8956 \\
%\hline
%{Few-Shot Audio} & 0.4588 & \textbf{0.8930} & \textbf{0.9449} \\
%\hline
%{Ours} & \textbf{0.4906} & 0.8319 & 0.9137 \\
\end{tabular}
\label{image_audio_weak}
\vspace{-0mm}
\end{table*}

==> CVPR2021_Meta Alignment/tables/overview.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[t]
\fontsize{9}{11}\selectfont
\centering
\vspace{-0mm}
\caption{Data requirements for generalization (i.e. (meta)-test) in a target modality where both data and labels are rare. Cross-modal generalization leverages data from abundant source modalities for low-resource target modalities, requiring only a \textit{few samples} and \textit{no labels} in the target beyond those used for few-shot fine-tuning.}
\vspace{-1em}
\setlength\tabcolsep{2.0pt}
\begin{tabular}{l || c c c}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{\sc Approaches} & \multicolumn{3}{c}{\sc (Meta-)Train} \\
& Modality & Data & Labels \\
\Xhline{0.5\arrayrulewidth}
Transfer learning~\cite{baevski2019effectiveness} & Target & Many & None\\
\Xhline{0.5\arrayrulewidth}
Unsupervised pre-training~\cite{devlin2018bert} & Target & Many & None\\
Unsupervised meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} & Target & Many & None\\
\Xhline{0.5\arrayrulewidth}
%\makecell[l]{Within modality generalization\\(e.g. meta-learning~\cite{finn2017model,nichol2018reptile},\\transfer learning~\cite{DBLP:journals/corr/HuhAE16},\\domain adaptation~\cite{DBLP:journals/corr/TzengHSD17})} & Target & Many & Many & Target & Few & Few\\
Domain adaptation~\cite{tzeng2017adversarial} & Target & Many & Many\\
Few-shot learning~\cite{finn2017model} & Target & Many & Many\\
\Xhline{0.5\arrayrulewidth}
\multirow{2}{*}{\parbox{4.5cm}{Within modality + cross-modal learning~\cite{DBLP:journals/corr/abs-1903-11101,10.5555/2999611.2999716,DBLP:journals/corr/abs-1710-08347,NIPS2019_8731,zadeh2020foundations}}} & Source & Many & None \\
& Target & Many & Many \\
\Xhline{0.5\arrayrulewidth}
\multirow{2}{*}{\textbf{Cross-modal generalization (ours)}} & Source & Many & Many \\
& \textbf{Target} & \textbf{Few} & \textbf{None} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{overview_table}
\vspace{-4mm}
\end{table}

\iffalse
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[t]
\fontsize{9}{11}\selectfont
\centering
\vspace{-6mm}
\caption{Data requirements for generalization in a scarce target modality where both data and labels are rare. We use (meta-)train and (meta-)test to generalize conventional train and test stages in order to emphasize the availability of data and labels in the source and target. Cross-modal generalization leverages data from abundant source modalities for low-resource target modalities, thereby requiring only a \textit{few samples} and \textit{no labels} in the target beyond those used for few-shot fine-tuning.}
\setlength\tabcolsep{2.0pt}
\begin{tabular}{l || c c c c c c}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{\sc Approaches} & \multicolumn{3}{c}{\sc (Meta-)Train} & \multicolumn{3}{c}{\sc (Meta-)Test} \\
& Modality & Data & Labels & Modality & Data & Labels\\
\Xhline{0.5\arrayrulewidth}
{Transfer learning/Pre-training~\cite{baevski2019effectiveness,devlin2018bert}} & Target & Many & None & Target & Few & Few\\
\Xhline{0.5\arrayrulewidth}
Unsupervised meta-learning~\cite{DBLP:journals/corr/abs-1810-02334} & Target & Many & None & Target & Few & Few\\
\Xhline{0.5\arrayrulewidth}
%\makecell[l]{Within modality generalization\\(e.g. meta-learning~\cite{finn2017model,nichol2018reptile},\\transfer learning~\cite{DBLP:journals/corr/HuhAE16},\\domain adaptation~\cite{DBLP:journals/corr/TzengHSD17})} & Target & Many & Many & Target & Few & Few\\
Domain adaptation, Few-shot learning~\cite{finn2017model,tzeng2017adversarial} & Target & Many & Many & Target & Few & Few\\
\Xhline{0.5\arrayrulewidth}
\multirow{2}{*}{\parbox{5.1cm}{Within modality generalization + cross-modal learning~\cite{DBLP:journals/corr/abs-1903-11101,10.5555/2999611.2999716,DBLP:journals/corr/abs-1710-08347,NIPS2019_8731,zadeh2020foundations}}} & Source & Many & None & \multirow{2}{*}{Target} & \multirow{2}{*}{Few} & \multirow{2}{*}{Few}\\
& Target & Many & Many \\
\Xhline{0.5\arrayrulewidth}
\multirow{2}{*}{\textbf{Cross-modal generalization (this work)}} & Source & Many & Many & \multirow{2}{*}{\textbf{Target}} & \multirow{2}{*}{\textbf{Few}} & \multirow{2}{*}{\textbf{Few}}\\
& \textbf{Target} & \textbf{Few} & \textbf{None} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{overview_table}
\vspace{-4mm}
\end{table}
\fi

==> CVPR2021_Meta Alignment/tables/recipe_params.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\centering
\caption{Table of hyperparameters for generalization experiments on text to image task. Batchsize $4/8/16$ indicates the batchsize used for $1/5/10$-shot experiments respectively.\vspace{2mm}}
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{14}{*}{Text Encoder}
& Shared layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-3$\\
& Iterations & $800$\\
& Number of evaluation tasks & 16\\
& Loss Margin & $0.1$\\
& Width Factor & $1.3$ \\
& Number of Layers & $4$ \\
& Blocks Per Layer & $4, 5, 24, 3$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{14}{*}{Image Encoder}
& Shared layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-3$\\
& Iterations & $800$\\
& Number of evaluation tasks & 16\\
& Loss Margin & $0.1$\\
& Intermediate Pooling Function & Max \\
& Final Pooling Function & Average \\
& Stride & 1 \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{13}{*}{Image Classifier}
& Num hidden layers & $1$ \\
& Hidden layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-3$\\
& Iterations & $800$\\
& Number of evaluation tasks & 16\\
& Loss & MSE\\
& Teacher forcing rate & $0.5$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-4mm}
\label{recipe_params}
\end{table}

==> CVPR2021_Meta Alignment/tables/tts.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[t]
\fontsize{9}{11}\selectfont
\centering
\caption{Language classification predictions on low-resource speech samples after training on labeled text data. Despite seeing just $5$ labeled speech samples, our method is able to accurately classify low-resource languages.\vspace{-1em}}
\setlength\tabcolsep{4.0pt}
\begin{tabular}{l || c c c c c c}
\Xhline{3\arrayrulewidth}
{\sc Speech (text in parenthesis)} & {\sc Oracle} & {\sc \names\ (ours)}\\
\Xhline{0.5\arrayrulewidth}
% 1 6
(Beda Yesus agot gu ofa oida Bua buroru Didif ojgomu) & {\color{rr} Russian} & {\color{gg} Meax} \\
% 7 0 
%(Jesus pu ayan tyaateexaa tijin)    & {\color{gg} Cora} & {\color{rr} Jamaican Patois} \\
% 2 0
%(Goliyi ri ta isuli ki ni ri iyi aziazi yi aado ta isuisu anya be)  & {\color{gg} Avokaya} & {\color{rr} Jamaican Patois} \\
% 8 0
(Ido hai Timotiu natile hampai moula Aturana Musa) & {\color{rr} Jamaican Patois} & {\color{gg} Badaic} \\
% 3 2
(Mu habotu pa kali Mataoqu osolae vekoi Rau sari Mua kana pa kauru Nenemu gua) & {\color{rr} Avokaya} & {\color{gg} Roviana}\\
% 3 3   (8)
%(Hangko inditi Paulu hai rangana meangka mbulimohe) & {\color{rr} Roviana} & {\color{rr} Roviana} \\
% 2 4   (4)
%(Laha tui shei thunq de iwn shei de la athi kkrhau jo de)   & {\color{rr} Avokaya} & {\color{gg} Mro} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{samples}
\vspace{-4mm}
\end{table*}


\iffalse
\begin{table}[]
\caption{Text-Speech Results: no\_meta\_tri is our proposed approach without any meta learning, meta\_1\_tri is our proposed approach with meta learning applied to only the classifier, reptile\_audio is unimodal meta learning, reptile\_cos is our proposed approach with our alignment loss function replaced with the cosine similarity loss, reptile\_tri is our proposed approach that uses triplet loss, lstm\_ae is the unsupervised unimodal model}
\begin{tabular}{lrr}
                   & \multicolumn{1}{l}{mean} & \multicolumn{1}{l}{stdev} \\
no\_meta\_tri k1   & 0.09713                  & 0.05298687573             \\
no\_meta\_tri k5   & 0.0934                   & 0.04360081549             \\
no\_meta\_tri k10  & 0.18798                  & 0.1472042104              \\
meta\_1\_tri k1    & 0.09713                  & 0.05298687573             \\
meta\_1\_tri k5    & 0.0934                   & 0.04360081549             \\
meta\_1\_tri k10   & 0.18798                  & 0.1472042104              \\
reptile\_audio k1  & 0.26864                  & 0.08181976398             \\
reptile\_audio k5  & 0.42367                  & 0.2679192791              \\
reptile\_audio k10 & 0.89423                  & 0.2588449474              \\
reptile\_cos k1    & 0.2119                   & 0.04135940038             \\
reptile\_cos k5    & 0.675                    & 0.2898754522              \\
reptile\_cos k10   & 0.64375                  & 0.4497781089              \\
reptile\_tri k1    & 0.38066                  & 0.08024892107             \\
reptile\_tri k5    & 0.42019                  & 0.1280220593              \\
reptile\_tri k10   & 0.40937                  & 0.2181009606              \\
lstm\_ae k1        & 0.1546666667             & 0.04751971521             \\
lstm\_ae k5        & 0.1827                   & \multicolumn{1}{l}{-}     \\
lstm\_ae k10       & 0.3353                   & \multicolumn{1}{l}{-}    
\end{tabular}
\end{table}
\fi

==> CVPR2021_Meta Alignment/tables/tts_da.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[t]
\fontsize{9}{11}\selectfont
\centering
\caption{Performance on text to speech generalization on the Wilderness dataset. We compare \name\ with some standard domain adaptation baselines and observe that none of them perform well on cross-modal generalization. Although domain confusion and alignment do improve upon standard encoder sharing, they still fall short of our approach. This serves to highlight the empirical differences between cross-modal generalization and domain adaptation.}
\setlength\tabcolsep{2.0pt}
\begin{tabular}{l l || c c c c c c}
\Xhline{3\arrayrulewidth}
{\sc Type} & {\sc Approach}  & {\sc 1-Shot} & {\sc 5-Shot} & {\sc 10-Shot} & {\sc \#Speech (labeled)}\\
\Xhline{0.5\arrayrulewidth}
\multirow{4}{*}{Domain Adaptation} & Shared & $55.6 \pm 10.2$ & $75.2 \pm 8.4$ & $81.9 \pm 3.9$ & $4395 (0)$\\
& Shared + Align~\cite{jawanpuria2020geometry} & $59.7 \pm 7.6$ & $78.4 \pm 6.2$ & $84.3 \pm 1.5$ & $4395 (0)$\\
& Shared + Domain confusion~\cite{DBLP:journals/corr/TzengHZSD14} & $59.5 \pm 7.2$ & $76.3 \pm 9.4$ & $83.9 \pm 1.8$ & $4395 (0)$\\
& Shared + Target labels~\cite{DBLP:journals/corr/abs-0907-1815} & $57.3 \pm 9.3$ & $76.2 \pm 8.4$ & $84.0 \pm 1.9$ & $4395 (4395)$\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{Cross-modal} & Align + Classify~\cite{cicek2019unsupervised,DBLP:journals/corr/abs-1711-03213,DBLP:journals/corr/RajNT15a,tzeng2017adversarial,10.5555/2283516.2283652} & $61.1 \pm 6.0$ & $74.8 \pm 2.1$ & $86.2 \pm 0.7$ & $4395 (0)$\\
& Align + Meta Classify~\cite{sahoo2019metalearning} & $65.6 \pm 6.1$ & $89.9 \pm 1.5$ & $93.0 \pm 0.5$ & $4395 (0)$\\
& \textbf{\names\ (ours)} & $\mathbf{67.9 \pm 6.6}$ & $\mathbf{90.6 \pm 1.5}$ & $\mathbf{93.2 \pm 0.2}$ & $4395 (0)$\\
\Xhline{0.5\arrayrulewidth}
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{tts_da}
\vspace{-2mm}
\end{table*}

==> CVPR2021_Meta Alignment/tables/tts_params.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\centering
\caption{Table of hyperparameters for generalization experiments on text to speech task. Batchsize $4/8/16$ indicates the batchsize used for $1/5/10$-shot experiments respectively.\vspace{2mm}}
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{14}{*}{Text Encoder}
& Bidirectional & True \\
& Embedding dim & $256$ \\
& Num hidden layers & $1$ \\
& Hidden layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-4$\\
& Iterations & $800$\\
& Loss Margin & $0.1$\\
& Number of evaluation tasks & $16$\\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{13}{*}{Speech Encoder}
& Embedding dim & $40$ \\
& Num hidden layers & $2$ \\
& Hidden layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-4$\\
& Iterations & $800$\\
& Loss Margin & $0.1$\\
& Number of evaluation tasks & $16$\\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{13}{*}{Speech Classifier}
& Num hidden layers & $1$ \\
& Hidden layer size & $256$ \\
& Batchsize & $4/8/16$ \\
& Activation & ReLU \\
& Meta Optimizer & SGD \\
& Optimizer & Adam \\
& Meta Learning rate & $1e-1$ \\
& Align Learning rate & $1e-3$ \\
& Classifier Learning rate & $1e-4$\\
& Iterations & $800$\\
& Loss & MSE\\
& Teacher forcing rate & $0.5$ \\
& Number of evaluation tasks & $16$\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-0mm}
\label{tts_params}
\end{table}
